Exact Method of Moments for multi-dimensional population balance equations

The unique properties of anisotropic and composite particles are increasingly being leveraged in modern particulate products. However, tailored synthesis of particles characterized by multi-dimensional dispersed properties remains in its infancy and few mathematical models for their synthesis exist. Here, we present a novel, accurate and highly efficient numerical approach to solve a multi-dimensional population balance equation, based on the idea of the exact method of moments for nucleation and growth \cite{pflug2020emom}. The transformation of the multi-dimensional population balance equation into a set of one-dimensional integro-differential equations allows us to exploit accurate and extremely efficient numerical schemes that markedly outperform classical methods (such as finite volume type methods) which is outlined by convergence tests. Our approach not only provides information about complete particle size distribution over time, but also offers insights into particle structure. The presented scheme and its performance is exmplified based on coprecipitation of nanoparticles. For this process, a generic growth law is derived and parameter studies as well as convergence series are performed.

==> header.tex <==
\usepackage{lineno}
\usepackage{mathtools}
%% \biboptions{comma,round}
\newcommand{\xn}{x_\mathrm{n}}
\newcommand{\dd}{\, \mathrm d}
\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cG}{\mathcal G}
\newcommand{\cS}{\mathcal S}
\newcommand{\cC}{\mathcal C}
\newcommand{\sC}{\boldsymbol{\mathsf C}}
\newcommand{\brho}{\boldsymbol\rho}
\newcommand{\cH}{\mathcal H}
\newcommand{\cN}{\mathcal N}
\newcommand{\cM}{\mathcal M}
\newcommand{\x}{\boldsymbol x}
\newcommand{\y}{\boldsymbol y}
\newcommand{\bdelta}{{\boldsymbol \delta}}
\newcommand{\cc}{{\boldsymbol c}}
\newcommand{\CC}{{\boldsymbol C}}
%\newcommand{\hxxi}{{\boldsymbol{\hat \xi}}}

\newcommand{\hxxiC}{\boldsymbol{\hat \xi^{\mathsf C}}}
\newcommand{\hxxiCo}{\boldsymbol{\hat \xi^{\mathsf C}}_{\!\!\!\!\!1}\,}
\newcommand{\hxxiCt}{\boldsymbol{\hat \xi^{\mathsf C}}_{\!\!\!\!\!2}\,}

\newcommand{\xxxic}{\boldsymbol{\xi^{\mathsf c}}}
\newcommand{\xxxico}{\boldsymbol{\xi^{\mathsf c}}_{\!\!\!1}}
\newcommand{\xxxict}{\boldsymbol{\xi^{\mathsf c}}_{\!\!\!2}}

\newcommand{\txxxic}{\boldsymbol{\tilde \xi^{\mathsf c}}}
\newcommand{\txxxico}{\boldsymbol{\tilde \xi^{\mathsf c}}_{\negthickspace\negthickspace 1}}
\newcommand{\txxxict}{\boldsymbol{\tilde \xi^{\mathsf c}}_{\negthickspace\negthickspace 2}}

\newcommand{\mX}{{\boldsymbol{\mathcal X}}}
%\newcommand{\txxi}{{\boldsymbol{\tilde \xi}}}
%\newcommand{\llambda}{\boldsymbol \lambda}
%\newcommand{\xxi}{\boldsymbol \xi}
%\newcommand{\xxic}{\boldsymbol{\xi^c}}
%\newcommand{\txxic}{\boldsymbol{\tilde \xi^c}} 
\newcommand{\ccG}{\boldsymbol \cG}
\newcommand{\ggamma}{\boldsymbol \gamma}
\newcommand{\oomega}{\boldsymbol \omega}
\newcommand{\m}{\boldsymbol m}
\newcommand{\V}{\boldsymbol V\!}
\newcommand{\GG}{\boldsymbol G}
\newcommand{\ct}{\boldsymbol t}
\newcommand{\cv}{\boldsymbol v}
%\newcommand{\tcG}{\tilde{\mathcal G}}
%\newcommand{\tcN}{\tilde{\mathcal N}}
\renewcommand{\:}{\mathrel{\coloneqq}}
\renewcommand{\=}{\ensuremath{\eqqcolon}}
\newcommand{\equivd}{\ensuremath{\vcentcolon\equiv}}
% \biboptions{}
\newcommand{\todoA}[1]{\todo[inline,color=green!30!white]{Adeel: #1}}
\newcommand{\todoL}[1]{\todo[inline,color=yellow!40!white]{Lukas: #1}}
\newcommand{\todoT}[1]{\todo[inline,color=blue!40!white]{Tobi: #1}}
\newcommand{\todoLT}[1]{\todo[inline,color=red!40!white]{Lukas und Tobi: #1}}
\theoremstyle{plain}


\newtheorem{ass}[theorem]{Assumption}
\newtheorem{defi}[theorem]{Definition}
\newtheorem{prob}[theorem]{Problem statement}
\newtheorem*{exa}{Example}
\newtheorem*{algo}{Algorithm}
\newtheorem{cor}[theorem]{Corollary}

\newtheoremstyle{boldremark}
    {\dimexpr\topsep/2\relax} % space above
    {\dimexpr\topsep/2\relax} % space below
    {}          % body font
    {}          % indent amount
    {\bfseries\itshape} % theorem head font
    {.}         % punctuation after theorem head
    {.5em}      % space after theorem head
    {}          % theorem hed spec. (empty = "normal")
\theoremstyle{boldremark}    
\usepackage{tikz}
\usetikzlibrary{shapes,arrows,positioning}
\usepackage[nameinlink]{cleveref}

==> header_elsarticle.tex <==
\usepackage{lineno}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}
%% \biboptions{comma,round}
\newcommand{\xn}{x_\mathrm{n}}
\newcommand{\dd}{\, \mathrm d}
\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cG}{\mathcal G}
\newcommand{\cS}{\mathcal S}
\newcommand{\cC}{\mathcal C}
\newcommand{\sC}{\boldsymbol{\mathsf C}}
\newcommand{\brho}{\boldsymbol\rho}
\newcommand{\cH}{\mathcal H}
\newcommand{\cN}{\mathcal N}
\newcommand{\cM}{\mathcal M}
\newcommand{\x}{\boldsymbol x}
\newcommand{\y}{\boldsymbol y}
\newcommand{\bdelta}{{\boldsymbol \delta}}
\newcommand{\cc}{{\boldsymbol c}}
\newcommand{\CC}{{\boldsymbol C}}
%\newcommand{\hxxi}{{\boldsymbol{\hat \xi}}}

\newcommand{\hxxiC}{\boldsymbol{\hat \xi^{\mathsf C}}}
\newcommand{\hxxiCo}{\boldsymbol{\hat \xi^{\mathsf C}}_{\!\!\!\!\!1}\,}
\newcommand{\hxxiCt}{\boldsymbol{\hat \xi^{\mathsf C}}_{\!\!\!\!\!2}\,}

\newcommand{\xxxic}{\boldsymbol{\xi^{\mathsf c}}}
\newcommand{\xxxico}{\boldsymbol{\xi^{\mathsf c}}_{\!\!\!1}}
\newcommand{\xxxict}{\boldsymbol{\xi^{\mathsf c}}_{\!\!\!2}}

\newcommand{\txxxic}{\boldsymbol{\tilde \xi^{\mathsf c}}}
\newcommand{\txxxico}{\boldsymbol{\tilde \xi^{\mathsf c}}_{\negthickspace\negthickspace 1}}
\newcommand{\txxxict}{\boldsymbol{\tilde \xi^{\mathsf c}}_{\negthickspace\negthickspace 2}}

\newcommand{\mX}{{\boldsymbol{\mathcal X}}}
%\newcommand{\txxi}{{\boldsymbol{\tilde \xi}}}
%\newcommand{\llambda}{\boldsymbol \lambda}
%\newcommand{\xxi}{\boldsymbol \xi}
%\newcommand{\xxic}{\boldsymbol{\xi^c}}
%\newcommand{\txxic}{\boldsymbol{\tilde \xi^c}} 
\newcommand{\ccG}{\boldsymbol \cG}
\newcommand{\ggamma}{\boldsymbol \gamma}
\newcommand{\oomega}{\boldsymbol \omega}
\newcommand{\m}{\boldsymbol m}
\newcommand{\V}{\boldsymbol V\!}
\newcommand{\GG}{\boldsymbol G}
\newcommand{\ct}{\boldsymbol t}
\newcommand{\cv}{\boldsymbol v}
%\newcommand{\tcG}{\tilde{\mathcal G}}
%\newcommand{\tcN}{\tilde{\mathcal N}}
\renewcommand{\:}{\mathrel{\coloneqq}}
\renewcommand{\=}{\ensuremath{\eqqcolon}}
\newcommand{\equivd}{\ensuremath{\vcentcolon\equiv}}
% \biboptions{}
\newcommand{\todoA}[1]{\todo[inline,color=green!30!white]{Adeel: #1}}
\newcommand{\todoL}[1]{\todo[inline,color=yellow!40!white]{Lukas: #1}}
\newcommand{\todoT}[1]{\todo[inline,color=blue!40!white]{Tobi: #1}}
\newcommand{\todoLT}[1]{\todo[inline,color=red!40!white]{Lukas und Tobi: #1}}
%\theoremstyle{plain}

\newtheorem{thm}{Theorem} 
\newtheorem{lem}[thm]{Lemma} 
\newdefinition{defi}{Definition}

\usepackage{tikz}
\usetikzlibrary{shapes,arrows,positioning}
\usepackage[nameinlink]{cleveref}
